Visualizing Large-scale and High-dimensional Data

We study the problem of visualizing large-scale and high-dimensional data in a low-dimensional (typically 2D or 3D) space. Much success has been reported recently by techniques that first compute a similarity structure of the data points and then project them into a low-dimensional space with the structure preserved. These two steps suffer from considerable computational costs, preventing the state-of-the-art methods such as the t-SNE from scaling to large-scale and high-dimensional data (e.g., millions of data points and hundreds of dimensions). We propose the LargeVis, a technique that first constructs an accurately approximated K-nearest neighbor graph from the data and then layouts the graph in the low-dimensional space. Comparing to t-SNE, LargeVis significantly reduces the computational cost of the graph construction step and employs a principled probabilistic model for the visualization step, the objective of which can be effectively optimized through asynchronous stochastic gradient descent with a linear time complexity. The whole procedure thus easily scales to millions of high-dimensional data points. Experimental results on real-world data sets demonstrate that the LargeVis outperforms the state-of-the-art methods in both efficiency and effectiveness. The hyper-parameters of LargeVis are also much more stable over different data sets.

==> gConstruction__Jian_Tang_s_conflicted_copy_2015-10-12_.tex <==
\section{Approximate K-nearest Neighbor Graph Construction}
\label{sec::knn}
In this section, we introduce our proposed approach for constructing the approximate K-nearest neighbor graph. Given a set of high-dimensional data $\{\vec{x}_i\}_{i=1,\ldots, N}$, in which $\vec{x}_i \in R^d$, the naive way of constructing the K-nearest neighbor graph takes $O(N^2d)$ time, which is too costly for large-scale data. In literature, various indexing techniques have been proposed for approximate K-nearest neighbor construction such as space-partitioning trees (e.g., k-d tree~\cite{bentley1975multidimensional}, vantage-point tree~\cite{yianilos1993data}, random projection trees~\cite{dasgupta2008random}), locality sensitive hashing based techniques~\cite{datar2004locality}, and other technique based on neighbor exploring (e.g., NN-Descent~\cite{dong2011efficient}). 

%The approaches of space-partitioning trees partition the entire space into different regions and organize different regions into tree structures. The approaches of partitioning the space can be recursively done along an axis (e.g., k-d tree) or a random direction  (e.g., random projection trees). The locality sensitive hashing based methods hash the data points into different buckets, and data in the same buckets are similar to each other.  The K-d tree can accurately construct the K-nearest neighbor graph, however, it is only efficient on data sets with small dimension. The random projection trees and locality sensitive hashing is applicable for data with large dimension, but will become very inefficient in order to get a very high recall. 

In this paper, we propose a new approach for constructing approximate K-nearest neighbor graph through a combination of the random projection trees and neighbor exploring techniques.  The random projection trees recursively partition the whole space and build up a tree. For every non-leaf node of the tree, the technique selects a random hyperplane to split the space into two spaces, which become the children of the node. It first randomly select two points from the space corresponding to the non-leaf node and then take the hyperplane, which is equally distant to the two points.  In practice we can build multiple trees to improve the precision in finding k-nearest neighbors. To construct the approximate k-nearest neighbor graphs, for each data point, we can traversal these trees to find the candidates of the nearest neighbors. 

To construct a very accurate k-nearest neighbor graph, in practice we find that many trees have to be built, which significantly affects the efficiency of the algorithm. Instead of building a large number of trees to obtain an accurate k-nearest neighbor graph, we propose to use the neighbor exploring techniques to improve the accuracy of a less accurate k-nearest neighbor graph. The basic idea is that ``a neighbor of a neighbor is also likely to be a neighbor''~\cite{dong2011efficient}. In the beginning, we can use a few trees to construct a k-nearest neighbor graph, the accuracy of which may be not so high. Then for each node of the graph, we can retrieve the neighbors of the neighbors as the nearest neighbor candidate. We can repeatedly do this. In practice, we find that one iteration is enough to significantly improve the accuracy of the k-nearest neighbor graph.

%Specifically, we first use the random projection trees to construct an approximate K-nearest neighbor graph, which has a low recall. If we do not require the recall of the K-nearest neighbor graph to be high, the approach of random projection trees is very efficient. Once the approximate K-nearest neighbor graph is constructed, we move to refine the K-nearest neighbor graph. Based on the idea that ``a neighbor of a neighbor is also likely to be a neighbor'' used by NN-Descent~\cite{}, for data point, we explore the neighbors of neighbors as the candidates. We recursively do this for several times, which turns out to be very effectively and efficiently. Finally, we summarize our algorithm in Algo.~\ref{algo::K-NNG}

% introduce how to select the number of neighbors, the perplexity metric here ....



==> gConstruction_old.tex <==
\section{Approximate K-nearest Neighbor Graph Construction}
\label{sec::knn}
In this section, we introduce our proposed approach for constructing the approximate K-nearest neighbor graph. Given a set of high-dimensional data $\{\vec{x}_i\}_{i=1,\ldots, N}$, in which $\vec{x}_i \in R^d$, the naive way of constructing the K-nearest neighbor graph takes $O(N^2d)$ time, which is too costly for large-scale data. In literature, various indexing techniques have been proposed for approximate K-nearest neighbor construction such as space-partitioning trees (e.g., k-d tree~\cite{bentley1975multidimensional}, vantage-point tree~\cite{yianilos1993data}, random projection trees~\cite{dasgupta2008random}), locality sensitive hashing based techniques~\cite{datar2004locality}, and other technique based on neighbor exploring (e.g., NN-Descent~\cite{dong2011efficient}). 

%The approaches of space-partitioning trees partition the entire space into different regions and organize different regions into tree structures. The approaches of partitioning the space can be recursively done along an axis (e.g., k-d tree) or a random direction  (e.g., random projection trees). The locality sensitive hashing based methods hash the data points into different buckets, and data in the same buckets are similar to each other.  The K-d tree can accurately construct the K-nearest neighbor graph, however, it is only efficient on data sets with small dimension. The random projection trees and locality sensitive hashing is applicable for data with large dimension, but will become very inefficient in order to get a very high recall. 

% % % % explain random projection trees in detail here and the neighbor exploring procedure here % % % %
We use random projection trees as our basic technique .....

we propose a new approximate K-nearest neighbor graph construction algorithm based on the combination of random projection trees and the neighbor exploring technique in NN-Descent. Random projection trees 

Specifically, we first use the random projection trees to construct an approximate K-nearest neighbor graph, which has a low recall. If we do not require the recall of the K-nearest neighbor graph to be high, the approach of random projection trees is very efficient. Once the approximate K-nearest neighbor graph is constructed, we move to refine the K-nearest neighbor graph. Based on the idea that ``a neighbor of a neighbor is also likely to be a neighbor'' used by NN-Descent~\cite{}, for data point, we explore the neighbors of neighbors as the candidates. We recursively do this for several times, which turns out to be very effectively and efficiently. Finally, we summarize our algorithm in Algo.~\ref{algo::K-NNG}


==> related__JianTangPC_s_conflicted_copy_2015-09-26_.tex <==
\section{Related Work}
\label{sec::related}

\subsection{K-nearest Neighbor (KNN) Graph Construction}

Efficiently finding nearest neighbors is:

Random partition tree:  KD tree, VP tree:

Random projection tree:

LSH based approaches:

\subsection{Graph Visualization}


==> related__Jian_Tang_s_conflicted_copy_2015-09-30_.tex <==
\section{Related Work}
\label{sec::related}

Our work is mainly related to two categories of work: building K-nearest neighbor (KNN) graph and graph visualization. 

\subsection{K-nearest Neighbor (KNN) Graph Construction}

Building k-nearest neighbor graph is essential to many applications such as similarity search, collaborative filtering and machine learning methods such as manifold learning. The complexity of the naive approach through brute-force is $O(n^2d)$, in which $n$ is the number of data points and $d$ is the dimensionality of the data points. For data sets containing as many as millions of data points, it is too computationally expensive. To efficiently build the k-nearest neighbor graph, many approaches have been proposed, which can be classified into three categories: space partitioning trees, locality sensitive hashing and neighbor exploring.  

The approaches of space partitioning trees partition the entire space into different regions and organize them into tree structures such as the k-d tree~\cite{bentley1975multidimensional,friedman1977algorithm}, vp-tree~\cite{yianilos1993data} and cover trees~\cite{beygelzimer2006cover}.The k-d tree partitions the entire space into hyperrectangular cells through recursively splitting along one coordinate at a time; the vp tree 
recursively partitions the space through randomly picking a position (the ``vantage point'') in the space and then dividing the data points into two parts: one consists of points that are close to the vantage point within a threshold and the others are not. The partitioning tree based approaches can find exact neighbors. However, they are usually only effective for data with low dimensions and the performance significantly deteriorates when the dimension increases. To speed up the process for the high dimensional data, several variants of k-d trees have been proposed such as the randomized k-d trees~\cite{silpa2008optimised} and random projection trees~\cite{dasgupta2008random}. Instead of dividing the data points by splitting along coordinates, the approach of random projection trees splits the data along a random direction, which effectively addresses the problem caused by ``the curse of dimensionality". The partitioning trees are usually applicable for $l_2$ distance measures and do not naturally generalize to other distance or similarity measures. 

Another category of approaches are based on the locality sensitive hashing~\cite{datar2004locality}, which deploys multiple hashing functions to map the data points into different buckets and data points in the same buckets are close to each other. When searching for the closest data points, only the similarities between the query point and the data points in the same buckets as the query point are measured. The hashing based techniques can effectively scale up to large data sets and to data sets with high dimensionality. Different hashing functions have been designed for different distance measures such as $l_p$ with $p\in (0,2])$~\cite{datar2004locality}, cosine similarity~\cite{charikar2002similarity}, and hamming distance~\cite{gionis1999similarity}. 

Besides the above two types of approaches, their is an algorithm called NN-Descent~\cite{dong2011efficient}. The NN-Decent algorithm is based on the principle that ``a neighbor of a neighbor is also likely to be a neighbor''. Starting from a random K-NN graph, the NN-Descent algorithm repeatedly improves the approximation through exploring the neighbors' neighbors of each data point in the current approximation graph. The NN-Descent algorithm is applicable for generic similarity measures. However, the NN-Descent can only effectively search the accurate neighbors when the dimension of the data points is very small. When the dimension grows (>50), the recall significantly decreases.
     
Our proposed K-NN graph construction combines the techniques of random projection trees and the NN-Descent. We first use the random projection trees to build an approximate K-NN graph, the accuracy of which (e.g., 50\%) may be not so high but is still far better than the random K-NN graph used in the NN-Descent. Then we repeatedly improve the graph through exploring the neighbors of neighbors. We found that this hybrid approach scales up to data sets with large dimensionality and also has a very high recall. In the experiments, we empirically evaluate the effectiveness and efficiency of these approaches. 
  
\subsection{Graph Visualization}

The problem of graph visualization essentially aims to embed the graphs into two or three dimensional spaces. The goal is to make similar points be close to each other and dissimilar data points be far away from each other.
The classical approach include Isomap~\cite{tenenbaum2000global}, local linear embedding~\cite{roweis2000nonlinear}, Laplacian Eigenmaps~\cite{belkin2001laplacian}, stochastic neighbor embeddings (SNE)~\cite{hinton2002stochastic}. Though these technique have been proved to be very effective on artificial data sets, they do not perform so well in real-world high-dimensional data. Besides, all these techniques cannot scale up to large-scale data sets.

in which a Gaussian distribution is used to compute the similarities between the data points in the low-dimensional space. 

The SNE approach has two limitations. One is that it is very hard to optimize. Besides, it suffers from the problem of data crowding, i.e., many points are likely to crowd in the center of the map. To resolve these problems, Maaten and Hinton proposed the t-SNE.


